High-Energy Neutrino Astronomy: A Glimpse of the Promised Land

In 2012, physicists and astronomers celebrated the hundredth anniversary of the detection of cosmic rays by Viktor Hess. One year later, in 2013, there was first evidence for extraterrestrial high-energy neutrinos, i.e. for signal which may contain key information on the origin of cosmic rays. That evidence is provided by data taken with the IceCube neutrino telescope at the South Pole. First concepts to build a detector of this kind have been discussed at the 1973 International Cosmic Ray Conference. Nobody would have guessed at that time that the march towards first discoveries would take forty years, the biblical time of the march from Egypt to Palestine. But now, after all, the year 2013 has provided us a first glimpse to the promised land of the neutrino universe at highest energies. This article sketches the evolution towards detectors with a realistic discovery potential, describes the recent relevant results obtained with the IceCube and ANTARES neutrino telescopes and tries a look into the future.

==> styles/proc_def.tex <==
%------------------------------------------------------------------------------
%       Some special symbols etc.:
%       --------------------------
%       -> small numbers
%------------------------------------------------------------------------------
\def\zero{{\scriptscriptstyle 0}}
\def\sone{{\scriptscriptstyle 1}}
\def\stwo{{\scriptscriptstyle 2}}
\def\sthr{{\scriptscriptstyle 3}}
\def\sfou{{\scriptscriptstyle 4}}
\def\sfiv{{\scriptscriptstyle 5}}
\def\sfiv{{\scriptscriptstyle 5}}
\def\ssix{{\scriptscriptstyle 6}}
\def\ssev{{\scriptscriptstyle 7}}
\def\seig{{\scriptscriptstyle 8}}
\def\snin{{\scriptscriptstyle 9}}
\def\sten{{\scriptscriptstyle 10}}
\def\half{{\scriptscriptstyle 1/2}}
%------------------------------------------------------------------------------
%       -> define \coll and \etal macros used in
%          LaTeX4zeus bibliography data base
%------------------------------------------------------------------------------
\providecommand{\coll}{Coll.\xspace}
\providecommand{\colls}{Colls.\xspace}
\providecommand{\etal}{et al.\xspace}
%------------------------------------------------------------------------------
%       -> experiment, accelerator, lab names in \sc
%------------------------------------------------------------------------------
\newcommand{\expname}[1]{{\scshape #1}\xspace}
\newcommand{\AMANDA}{\expname{Amanda}}
\newcommand{\ANTARES}{\expname{Antares}}
\newcommand{\AMADEUS}{\expname{Amadeus}}
\newcommand{\BEBC}{\expname{Bebc}}
\newcommand{\CERN}{\expname{Cern}}
\newcommand{\DESY}{\expname{Desy}}
\newcommand{\FNAL}{\expname{Fnal}}
\newcommand{\HERA}{\expname{Hera}}
\newcommand{\KMNeT}{\expname{KM3NeT}}
\newcommand{\ICECUBE}{\expname{IceCube}}
\newcommand{\LHC}{\expname{Lhc}}
\newcommand{\NEMO}{\expname{Nemo}}
\newcommand{\NESTOR}{\expname{Nestor}}
\newcommand{\OPERA}{\expname{Opera}}
\newcommand{\TESLA}{\expname{Tesla}}
\newcommand{\THERA}{\expname{Thera}}
\newcommand{\ZEUS}{\expname{Zeus}}
%------------------------------------------------------------------------------
%       -> additional name operators
%------------------------------------------------------------------------------
\newcommand{\odiv}{{\operatorname*{div}}}
\newcommand{\ograd}{{\operatorname*{grad}}}
\newcommand{\orot}{{\operatorname*{rot}}}
\newcommand{\odiag}{{\operatorname*{diag}}}
%------------------------------------------------------------------------------
%       -> "unknown" and "none" markers
%------------------------------------------------------------------------------
\def\xxx{\hbox{$\qsm\qsm\qsm$}\xspace}
\def\none{---}
%------------------------------------------------------------------------------
%       -> Euro symbol
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\@ifundefined{euro}%
{\providecommand{\Euro}{Euro\xspace}
 \providecommand{\EURO}{\,Euro\xspace}}%
{\providecommand{\Euro}{\euro\xspace}
 \providecommand{\EURO}{\,\euro\xspace}}
\catcode`\@=12 % @ signs are no longer letters
%------------------------------------------------------------------------------
%       -> shorthands for particles
%------------------------------------------------------------------------------
\def\Wpm{{W^\pm}}
\def\Z0{{Z^\zero}}
%------------------------------------------------------------------------------
%       -> eV and multiples
%------------------------------------------------------------------------------
\def\eVdist{\kern-0.06667em}
\def\Ev{{\text{e}\eVdist\text{V\/}}}
\def\Kev{{\text{ke}\eVdist\text{V\/}}}
\def\Mev{{\text{Me}\eVdist\text{V\/}}}
\def\Gev{{\text{Ge}\eVdist\text{V\/}}}
\def\Tev{{\text{Te}\eVdist\text{V\/}}}
\def\Pev{{\text{Pe}\eVdist\text{V\/}}}
\def\Eev{{\text{Ee}\eVdist\text{V\/}}}
\def\Zev{{\text{Ze}\eVdist\text{V\/}}}
\def\ev{{\,\text{e}\eVdist\text{V\/}}}
\def\kev{{\,\text{ke}\eVdist\text{V\/}}}
\def\mev{{\,\text{Me}\eVdist\text{V\/}}}
\def\gev{{\,\text{Ge}\eVdist\text{V\/}}}
\def\tev{{\,\text{Te}\eVdist\text{V\/}}}
\def\pev{{\,\text{Pe}\eVdist\text{V\/}}}
\def\eev{{\,\text{Ee}\eVdist\text{V\/}}}
\def\zev{{\,\text{Ze}\eVdist\text{V\/}}}
%------------------------------------------------------------------------------
%       -> various other units (for math mode only)
%------------------------------------------------------------------------------
\def\pb{\,\text{nb}}
\def\pb{\,\text{pb}}
\def\fb{\,\text{fb}}
\def\pbi{\,\text{pb}^{-1}}
\def\fbi{\,\text{fb}^{-1}}
\def\met{\,\text{m}}
\def\Met{\text{m}}
\def\cm{\,\text{cm}}
\def\Cm{\text{cm}}
\def\mm{\,\text{mm}}
\def\km{\,\text{km}}
\def\Km{\text{km}}
\def\mum{\,\upmu\text{m}}
\def\nm{\,\text{nm}}
\def\lit{\,\text{l}}
\def\mA{\,\text{mA}}
\def\Hz{\,\text{Hz}}
\def\kHz{\,\text{kHz}}
\def\MHz{\,\text{MHz}}
\def\GHz{\,\text{GHz}}
\def\ppm{\,\text{ppm}}
\def\hour{\,\text{h}}
\def\scnd{\,\text{s}}
\def\Scnd{\text{s}}
\def\musec{\,\upmu\text{s}}
\def\ns{\,\text{ns}}
\def\psec{\,\text{ps}}
\def\years{\,\text{a}}
\def\mets{\,\text{m}/\text{s}}
\def\cms{\,\text{cm}/\text{s}}
\def\rad{\,\text{rad}}
\def\mrad{\,\text{mrad}}
\def\murad{\,\upmu\text{rad}}
\def\gramm{\,\text{g}}
\def\kgramm{\,\text{kg}}
\def\Kgramm{\text{kg}}
\def\Tesla{\,\text{T}}
\def\Kelvin{\,\text{K}}
\def\Joule{\,\text{J}}
\def\kJoule{\,\text{kJ}}
\def\erg{\,\text{erg}}
\def\New{\,\text{N}}
\def\kNew{\,\text{kN}}
\def\Watt{\,\text{W}}
\def\kWatt{\,\text{kW}}
\def\Pascal{\,\text{Pa}}
\def\mPa{\,\text{mPa}}
\def\muPa{\,\upmu\text{Pa}}
\def\bar{\,\text{bar}}
\def\mol{\,\text{mol}}
\def\Mol{\text{mol}}
\def\Coul{\,\text{C}}
\def\Ampe{\,\text{A}}
\def\Volt{\,\text{V}}
\def\Ohm{\,\upOmega}
\def\kOhm{\,\text{k}\upOmega}
\def\Farad{\,\text{F}}
\def\pF{\,\text{pF}}
\def\nF{\,\text{nF}}
\def\muF{\,\upmu\text{F}}
\def\sr{\,\text{sr}}
\def\flunit{\gev\cm^{-2}\scnd^{-1}\sr^{-1}}
%------------------------------------------------------------------------------
%       -> commonly used symbols
%------------------------------------------------------------------------------
\def\Born{{\rm Born}}
\def\BR{{\rm BR}}
\def\CC{{\rm CC}}
\def\bCC{{\bf CC}}
\def\CI{{\rm CI}}
\def\CJ{{\rm CJ}}
\def\CL#1{$#1\%$~C.L\xdotspace}
\def\Cor{{\cal C}}
\def\D{{\rm d}}
\def\bD{{\bf d}}
\def\DA{{\scriptscriptstyle{\rm DA}}}
\def\DO{{D{\O}}\xspace}
\def\DCA{{\rm DCA}}
\def\F{{\cal F}}
\def\GRV{{\rm GRV}}
\def\IC{{\rm IC}}
\def\ISR{{\rm ISR}}
\def\IP{{\rm I$\kern-0.01667em$P}\xspace}
\def\JB{{\scriptscriptstyle{\rm JB}}}
\def\L{{\scriptscriptstyle{\rm L}}}
\def\LL{{\scriptscriptstyle{\rm LL}}}
\def\LQbar{\overline{\rm LQ}}
\def\LQsub{{\rm LQ}}
\def\LQ{{\rm LQ}}
\def\LR{{\scriptscriptstyle{\rm LR}}}
\def\Ldes{{\cal L}_{\rm des}}
\def\Lumi{{\cal L}}
\def\MC{{\rm MC}}
\def\MSbar{\hbox{$\overline{\rm MS}$}}
\def\NC{{\rm NC}}
\def\bNC{{\bf NC}}
\def\NS{{\rm NS}}
\def\Prob{{\cal P}}
\def\Ptlj{{\not{\kern-0.55ex P}}_t\ell j}
\def\Ptmiss{{\not{\kern-0.55ex P}}_t}
\def\QPM{{\rm QPM}}
\def\RL{{\scriptscriptstyle{\rm RL}}}
\def\RPv{{{\not R}_P}}
\def\RR{{\scriptscriptstyle{\rm RR}}}
\def\R{{\scriptscriptstyle{\rm R}}}
\def\SM{{\rm SM}}
\def\SMpCI{{\rm SM}+{\rm CI}}
\def\SUT{{\rm SU}(3)_c}
\def\SUTUO{{\rm SU}(2)_\L\times{\rm U}(1)_\Y}
\def\SUTSUTUO{{\rm SU}(3)_c\times{\rm SU}(2)_\L\times{\rm U}(1)_\Y}
\def\Ssup{{\rm S}}
\def\Y{{\scriptscriptstyle{\rm Y}}}
\def\alsmu#1{{\alpha_s(\mu_{#1}^2)}}
\def\alsmz{{\alpha_s(M_Z^2)}}
\def\alsqs{{\alpha_s(Q^2)}}
\def\als{\alpha_s}
\def\anti#1{\hbox{(anti-)}\discretionary{}{}{}#1}
\def\bkg{{\rm bkg}}
\def\cov{\text{cov}}
\def\ctwb{\cos\theta_W}
\def\ctws{\cos^2\theta_W}
\def\cut{{\rm cut}}
\def\data{{\rm data}}
\def\det{{\rm det}}
\def\dof{{\rm dof}}
\def\eff{{\rm eff}}
\def\elm{{\rm elm}}
\def\epslam{{\epsilon/\Lambda^2}}
\def\epslamz{{\epsilon/\Lambda^2_\zero}}
\def\evt{{\rm evt}}
\def\exc{{\rm exc}}
\def\fit{{\rm fit}}
\def\gh{{\gamma_h}}
\def\had{{\rm had}}
\def\jet{{\rm jet}}
\def\kg{{k_\gamma}}
\def\lsq#1{{\lambda_{#1}}}
\def\lsqp#1{{\lambda'_{#1}}}
\def\lsqpp#1{{{\lambda''}_{#1}}}
\def\meas{{\rm meas}}
\def\miss{{\rm miss}}
\def\obs{{\rm obs}}
\def\ord#1{{\cal O}(#1)}
\def\ordlr#1{{\cal O}\left(#1\right)}
\def\pnt{{\rm pnt}}
\def\rnge{{\,\text{--}\,}}
\def\rxsCC{\tilde\sigma^{e^+p\to\nubar_eX}}
\def\rxsNC{\tilde\sigma^{e^+p\to e^+X}}
\def\sMSbar{{\overline{\rm MS}}}
\def\sca{{\rm sca}}
\def\sexp{{\rm exp}}
\def\sihat{{\hat\sigma}}
\def\sint{{\rm int}}
\def\sarea{\text{\stru{0.5ex}{0.8ex} area}}
\def\seff{\text{\stru{1.5ex}{0.8ex} eff}}
\def\sevt{\text{\stru{0.5ex}{0.8ex} evt}}
\def\sgen{\text{\stru{0.5ex}{0.8ex} gen}}
\def\smin{\text{\stru{1.5ex}{0.2ex} min}}
\def\smax{\text{\stru{1.5ex}{0.2ex} max}}
\def\srad{{\rm rad}}
\def\sthe{{\rm the}}
\def\stwb{\sin\theta_W}
\def\stwss{\sin^4\theta_W}
\def\stws{\sin^2\theta_W}
\def\sys{{\rm sys}}
\def\ta{{\theta^\ast}}
\def\tilR{\tilde R}
\def\tilS{\tilde S}
\def\tilU{\tilde U}
\def\tilV{\tilde V}
\def\tileta{\tilde\eta}
\def\tl{{\theta_\ell}}
\def\tot{{\rm tot}}
\def\true{{\rm true}}
\def\tw{\theta_W}
\newcommand{\shto}{\ensuremath{\text{H$_2$O}}}
%------------------------------------------------------------------------------
%       nuclear symbols
%------------------------------------------------------------------------------
\newcommand{\nucl}[2]{\ensuremath{\stru{2.ex}{0.8ex}^{#2}{\rm #1}}}
\newcommand{\nuclz}[3]{\ensuremath{\,\stru{2.ex}{0.8ex}^{#2}_{#3}{\rm #1}}}
\newcommand{\nuclzn}[4]{\ensuremath{\stru{2.ex}{0.8ex}^{#2}_{#3}{\rm #1}
                        \stru{2.ex}{0.8ex}_{#4}}}
%------------------------------------------------------------------------------
%       -> some math symbols (+,-,...) for usage as mathchar's
%------------------------------------------------------------------------------
\mathchardef\qsm=63
\mathchardef\pls=43
\mathchardef\mns=512
\mathchardef\plm=518
\mathchardef\eql=61
\mathchardef\smallleft=300
\mathchardef\smallright=301
\mathchardef\perslsh=47
\mathchardef\les=316
\mathchardef\gre=318
\mathchardef\leq=532
\mathchardef\grq=533
%------------------------------------------------------------------------------
%       -> characters for typewriter font (used for http addresses)
%------------------------------------------------------------------------------
\chardef\amp=38
\chardef\usc=95
\chardef\til=126
%------------------------------------------------------------------------------
%       -> further special characters 
%------------------------------------------------------------------------------
\chardef\Lslash=138
%------------------------------------------------------------------------------
%       -> shorthand for "integral limits below and above"
%------------------------------------------------------------------------------
\def\intl{\int\limits}
\def\ointl{\oint\limits}
%------------------------------------------------------------------------------
%       -> footenote markers
%------------------------------------------------------------------------------
\def\fdag{$^{{\displaystyle\dagger})}$}
\def\fddag{$^{{\displaystyle\ddagger})}$}
\def\fstar{$^{{\displaystyle\star})}$}
\def\faste{$^{{\displaystyle\ast})}$}
%------------------------------------------------------------------------------
%       -> d'Alembert operator
%------------------------------------------------------------------------------
\def\sqr#1#2#3{{\vcenter{\hrule height.#3ex\hbox{\vrule width.#2ex height#1ex
    \kern#1ex\vrule width.#3ex}\hrule height.#2ex}}}
\def\dalem{\mathchoice\sqr{1.6}{08}{24}\sqr{1.6}{08}{24}
                      \sqr{1.4}{07}{21}\sqr{1.1}{06}{18}}
%------------------------------------------------------------------------------
%       -> rectangle with arrow ( '-> )
%------------------------------------------------------------------------------
\def\angleto{\vrule width.035em height2.1ex depth-.56ex\unskip\kern-.6ex\to}
%------------------------------------------------------------------------------
%       -> permille sign
%------------------------------------------------------------------------------
\def\perchc#1{{\raise.4ex\hbox{$\mkern4mu#1{\it\perslsh}_
             {\mkern-5mu\scriptscriptstyle{{\rm o}\!{\rm o}}}^
             {\mkern-12.8mu\scriptscriptstyle{\rm o}}$}}}
\def\permil{{\mathchoice\perchc{\displaystyle}\perchc{\textstyle}
             \perchc{\scriptstyle}\perchc{\scriptscriptstyle}}}
%------------------------------------------------------------------------------
%       -> wide bar and bar in parantheses as mathaccents, some applications
%------------------------------------------------------------------------------
\def\widebar#1{\mkern1.5mu\overline{\mkern-1.5mu#1\mkern-1.mu}\mkern1.mu}
\catcode`\@=11 % @ signs are now treated as letters
\def\parenbar{\mathpalette\p@renb@r}
\def\p@renb@r#1#2{\vbox{%
  \ifx#1\scriptscriptstyle \dimen@.7em\dimen@ii.2em\else
  \ifx#1\scriptstyle \dimen@.8em\dimen@ii.25em\else
  \dimen@1em\dimen@ii.4em\fi\fi \offinterlineskip
  \ialign{\hfill##\hfill\cr
    \vbox{\hrule width\dimen@ii}\cr
    \noalign{\vskip-.3ex}%
    \hbox to\dimen@{$\mathchar300\hfil\mathchar301$}\cr
    \noalign{\vskip-.3ex}%
    $#1#2$\cr}}}
\catcode`\@=12 % @ signs are no longer letters
\def\nuan{\parenbar{\nu}}
\def\ppbar{\parenbar{p}}
\def\qqbar{\parenbar{q}}
\def\ffbar{\parenbar{f}}
\def\pbar{\widebar{p}}
\def\nbar{\widebar{n}}
\def\qbar{\widebar{q}}
\def\dbar{\widebar{d}}
\def\ubar{\widebar{u}}
\def\sbar{\widebar{s}}
\def\cbar{\widebar{c}}
\def\bbar{\widebar{b}}
\def\tbar{\widebar{t}}
\def\fbar{\widebar{f}}
\def\nubar{\widebar{\nu}}
\def\Dbar{\widebar{D}}
\def\ebar{\widebar{e}}
\def\fbar{\widebar{f}}
\def\Ebar{\widebar{e}}
\def\Hebar{\widebar{\text{He}}}
\def\Cbar{\widebar{\text{C}}}
\def\Abar{\widebar{\text{A}}}
\def\Kbar{\widebar{K}}
\def\chibar{\widebar{\chi}}
\def\neulsp{{\tilde\chi_1^0}}
%------------------------------------------------------------------------------
%       Some shorthands and utilities:
%       ------------------------------
%       -> vertical rule of width zero and variable height & depth
%------------------------------------------------------------------------------
\newbox\struttbox
\setbox\struttbox=\hbox{\vrule height1.65ex depth.485ex width0pt}
\def\strutt{\relax\ifmmode\copy\struttbox\else\unhcopy\struttbox\fi}
\def\stru#1#2{\relax\ifmmode\hbox{\vrule height#1 depth#2 width0pt}
\else\vrule height#1 depth#2 width0pt\fi}
%------------------------------------------------------------------------------
%       -> underline with resonable distance text - line
%------------------------------------------------------------------------------
\def\uline#1{$\underline{\hbox{#1\strutt}}$}
%------------------------------------------------------------------------------
%       -> roman numbers (uppercase and lowercase)
%------------------------------------------------------------------------------
\def\ronum#1{\uppercase\expandafter{\romannumeral#1}}
\def\ronuml#1{\expandafter{\romannumeral#1}}
%------------------------------------------------------------------------------
%       -> vectors and matrices
%------------------------------------------------------------------------------
\def\vect#1{\begin{matrix}#1\end{matrix}}
\def\pvect#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bvect#1{\begin{bmatrix}#1\end{bmatrix}}
%------------------------------------------------------------------------------
%       -> some alignment tools for tables
%------------------------------------------------------------------------------
\def\cA{\ensuremath{{\phantom{0}}}}
\def\cB{\ensuremath{{\phantom{00}}}}
\def\cC{\ensuremath{{\phantom{000}}}}
\def\cD{\ensuremath{{\phantom{0000}}}}
\def\cM{\ensuremath{{\phantom{\mns}}}}
\def\cAm{\ensuremath{{\phantom{\mns0}}}}
\def\cBm{\ensuremath{{\phantom{\mns00}}}}
\def\cCm{\ensuremath{{\phantom{\mns000}}}}
\def\cDm{\ensuremath{{\phantom{\mns0000}}}}
\def\cCAAAC{\ensuremath{{\phantom{(000)}}}}
\def\cAd{\ensuremath{{\phantom{.0}}}}
\def\cBd{\ensuremath{{\phantom{0.0}}}}
\def\cbk{\kern-0.5em}
%------------------------------------------------------------------------------
%       -> shorthand for protected citations in captions and 
%          line breaks in headers
%------------------------------------------------------------------------------
\newcommand{\pcite}[1]{{\protect\cite{#1}}}
\def\pnl{\protect{\newline}}
%------------------------------------------------------------------------------
%       -> shorthands for equation, figure, table, section references
%------------------------------------------------------------------------------
\def\eq#1{(\ref{eq-#1})}
\def\eqsand#1#2{(\ref{eq-#1}) and~(\ref{eq-#2})}
\def\eqsto#1#2{(\ref{eq-#1})--(\ref{eq-#2})}
\def\eqstwo#1#2{(\ref{eq-#1},\ref{eq-#2})}
\def\eqsthr#1#2#3{(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3})}
\def\eqsfou#1#2#3#4{(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3},\ref{eq-#4})}
\def\Eq#1{Equation~(\ref{eq-#1})}
\def\Eqsto#1#2{Equations~(\ref{eq-#1})--(\ref{eq-#2})}
\def\fig#1{Fig.~\ref{fig-#1}}
\def\Fig#1{Figure~\ref{fig-#1}}
\def\figand#1#2{Figs.~\ref{fig-#1} and~\ref{fig-#2}}
\def\Figand#1#2{Figures~\ref{fig-#1} and~\ref{fig-#2}}
\def\tab#1{Table~\ref{tab-#1}}
\def\Tab#1{Table~\ref{tab-#1}}
\def\tabsand#1#2{Tables~\ref{tab-#1} and~\ref{tab-#2}}
\def\cha#1{Chap.~\ref{cha-#1}}
\def\Cha#1{Chapter~\ref{cha-#1}}
\def\sec#1{Sect.~\ref{sec-#1}}
\def\Sec#1{Section~\ref{sec-#1}}
\def\secand#1#2{Sects.~\ref{sec-#1} and~\ref{sec-#2}}
\def\secsto#1#2{Sects.~\ref{sec-#1} to~\ref{sec-#2}}
\def\Secand#1#2{Sections~\ref{sec-#1} and~\ref{sec-#2}}
\def\Secsto#1#2{Sections~\ref{sec-#1} to~\ref{sec-#2}}
\def\Abs#1{Abschnitt~\ref{sec-#1}}
\def\Abse#1#2{Abschnitte~\ref{sec-#1} und~\ref{sec-#2}}
\def\Absn#1#2{Abschnitten~\ref{sec-#1} und~\ref{sec-#2}}
%------------------------------------------------------------------------------
%       -> empty line and checkbox for forms
%------------------------------------------------------------------------------
\newcommand{\linebox}[2][3.ex]{\uline{\hbox to #2{\stru{#1}{0.pt}\hfil}}}
\newcommand{\checkbox}{$\square$\ \ }
%------------------------------------------------------------------------------
%       -> sequential numbering
%------------------------------------------------------------------------------
\newcounter{seqnum}
\setcounter{seqnum}{0}
\newcommand{\SQN}{\stepcounter{seqnum}\theseqnum}
\newcommand{\SQR}{\setcounter{seqnum}{0}}
%------------------------------------------------------------------------------
%       Log file messages
%       -----------------
%------------------------------------------------------------------------------
\def\LogMess#1{\typeout{^^J==> #1^^J}}
%------------------------------------------------------------------------------
%       Local laguage changes
%       ---------------------
%------------------------------------------------------------------------------
\def\german#1{\selectlanguage{german}#1\selectlanguage{american}}
%------------------------------------------------------------------------------
%       Redefine mathbf, define mathbfs (slanted bold)
%       ----------------------------------------------
%------------------------------------------------------------------------------
\DeclareMathAlphabet{\mathbf}{OT1}{cmr}{bx}{n}
\def\mb{\mathbf}
\DeclareMathAlphabet{\mathbfs}{OT1}{lcmss}{bx}{sl}
\def\mbs{\mathbfs}
%------------------------------------------------------------------------------
%       Additional functionality for tables and figures
%       -----------------------------------------------
%       prepare narrow figures in list environment
%------------------------------------------------------------------------------
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newlength\listtextwidth
\newcommand{\preparelistfloat}[1]{
  \setlength{\listtextwidth}{\textwidth}
  \addtolength{\listtextwidth}{-#1}}
%------------------------------------------------------------------------------
%       pseudo-footnotes for tables
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newlength{\@tabfninsert}
\newlength{\@tabfnwidth}
\newcommand{\tabfootnote}[2]{%
  \setlength{\@tabfninsert}{0.8em}
  \setlength{\@tabfnwidth}{\textwidth}
  \addtolength{\@tabfnwidth}{-\@tabfninsert}
  \addtolength{\@tabfnwidth}{-0.4em}
  \noindent\makebox[\@tabfninsert][r]{\footnotesize$^{#1}$\hfil}\hfill%
  \parbox[t]{\@tabfnwidth}{\footnotesize #2\hfill}}
\catcode`\@=12 % @ signs are no longer letters
%------------------------------------------------------------------------------
%       bold horizontal lines in tables (from IOP style,
%       bcline adapted(stolen) from mdwtab.sty)
%------------------------------------------------------------------------------
\newcommand{\boldarrayrulewidth}{1pt} 
\newcommand{\bs}{\noalign{\vspace{3pt plus1.5pt minus1pt}}}
\newcommand{\bsh}{\noalign{\vspace{2pt plus0.2pt minus0.5pt}}}
\newcommand{\bsn}{\noalign{\vspace{-0.5pt plus0.2pt minus0.2pt}}}
% Width of bold rule in tabular environment.
\catcode`\@=11 % @ signs are now treated as letters
\let\tab@penalty\relax
\newcount\tab@state
\def\bcline#1{%
  \noalign{\kern-.5\arrayrulewidth\tab@penalty}%
  \omit%
  \global\tab@state\@ne%
  \ranges\bcline@i{#1}%
  \cr%
  \noalign{\kern-.5\arrayrulewidth\tab@penalty}%
}
\def\bcline@i#1#2{%
  \ifnum#1<\tab@state\relax%
    \tab@@cr%
    \noalign{\kern-\arrayrulewidth\tab@penalty}%
    \omit%
    \global\tab@state\@ne%
  \fi%
  \@whilenum\tab@state<#1\do{%
    \hfil\tab@@tab@omit%
    \global\advance\tab@state\@ne%
  }%
  \ifnum\tab@state>\@ne%
    \kern-\arrayrulewidth%
  \fi%
  \@whilenum\tab@state<#2\do{%
    \tab@@span@omit%
    \global\advance\tab@state\@ne%
  }%
  \leaders\hrule\@height\boldarrayrulewidth\hfill%
}
\def\ranges#1#2{%
  \gdef\ranges@temp{#1}%
  \begingroup%
  \ranges@i#2 \q@delim%
}
\def\ranges@i{%
  \@ifnextchar\q@delim\ranges@done{\afterassignment\ranges@ii\count@}%
}
\def\ranges@ii{%
  \@ifnextchar-\ranges@iii{\ranges@do\count@\count@\ranges@v}%
}
\def\ranges@iii-{\afterassignment\ranges@iv\@tempcnta}
\def\ranges@iv{\ranges@do\count@\@tempcnta\ranges@v}
\def\ranges@v{%
  \@ifnextchar,%
    \ranges@vi%
    {%
      \@ifnextchar\q@delim%
        \ranges@done%
        {\tab@err@range\ranges@vi,}%
    }%
}
\def\ranges@vi,{\afterassignment\ranges@ii\count@}
\def\ranges@do#1#2{%
  \ifnum#1>#2\else%
    \expandafter\endgroup%
    \expandafter\ranges@temp%
    \expandafter{%
    \the\expandafter#1%
    \expandafter}%
    \expandafter{%
    \the#2%
    }%
    \begingroup%
  \fi%
}
\def\ranges@done\q@delim{\endgroup}
\def\ifinrange#1#2{%
  \@tempswafalse%
  \count@#1%
  \ranges\ifinrange@i{#2}%
  \if@tempswa%
    \expandafter\@firstoftwo%
  \else%
    \expandafter\@secondoftwo%
  \fi%
}
\def\ifinrange@i#1#2{%
  \ifnum\count@<#1 \else\ifnum\count@>#2 \else\@tempswatrue\fi\fi%
}
\def\tab@@cr{\cr}
\def\tab@@tab@omit{&\omit}
\def\tab@@span@omit{\span\omit}
\def\tab@checkrule#1{%
  \count@#1\relax%
  \expandafter\ifinrange%
  \expandafter\count@%
  \expandafter{\tab@xcols}%
    {\tab@checkrule@i}%
    {}%
}
\def\bhline{\noalign{\ifnum0=`}\fi\hrule \@height  
\boldarrayrulewidth \futurelet \@tempa\@xhline}
\def\@xhline{\ifx\@tempa\hline\vskip \doublerulesep\fi
      \ifnum0=`{\fi}}
\catcode`\@=12 % @ signs are no longer letters
% Rules for tables with extra space around
\newcommand{\topline}{\hline\bs}
\newcommand{\tophline}{\hline\bsh}
\newcommand{\topboldline}{\bhline\bs}
\newcommand{\midline}{\bs\hline\bs}
\newcommand{\midhline}{\bsh\hline\bsh}
\newcommand{\subheaderline}{\bs\hline\bsh}
\newcommand{\midboldline}{\bs\bhline\bs}
\newcommand{\bottomline}{\bs\hline}
\newcommand{\bottomhline}{\bsh\hline}
\newcommand{\bottomboldline}{\bs\bhline}
%------------------------------------------------------------------------------
%       extended functionality for figures: allow to add axodraw 
%       and picture items
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newcounter{pict@width}
\newcounter{pict@height}
\newlength{\pict@scale}
\setlength{\pict@scale}{0.1mm}
\newcommand{\psfigadd}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox to #2{\hspace{-\fill}\begin{picture}(\thepict@width,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#2,height=#3,clip=}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\newcounter{pict@widthfst}
\newcounter{pict@widthscd}
\newcounter{pict@widthtot}
\newcommand{\psfigaddtwo}[7]{%
\setcounter{pict@widthfst}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@widthscd}{1*\ratio{#2+#4+\pict@scale/2}{\pict@scale}}
\setcounter{pict@widthtot}{1*\ratio{#2+#4+#6+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\hspace{-\fill}\begin{picture}(\thepict@widthtot,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#2,height=#3,clip=}}
\put(\thepict@widthscd,0){\psfig{figure=#5,width=#6,height=#3,clip=}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#7}
\end{picture}}
}
\newcommand{\psfigror}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\begin{picture}(\thepict@width,\thepict@height)
\put(0,\thepict@height){\psfig{figure=#1,width=#3,height=#2,clip=,angle=270}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\newcommand{\psfigrol}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\begin{picture}(\thepict@width,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#3,height=#2,clip=,angle=90}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\catcode`\@=12 % @ signs are no longer letters

